Differential Cohomology as Diffeological Homotopy Theory

Thin homotopies, introduced by Caetano-Picken, serve to axiomatize the holonomy of connections on principal bundles. This approach has been generalized to higher non-abelian bundles with connection through transport functors and higher holonomies, at least in dimension two and partially in dimension three. In this thesis, we introduce a new variant of thin homotopy based on the definition of skeletal diffeologies introduced recently by Kihara and show that, in the abelian setting, ordinary differential cohomology can be completely recovered in terms of the homotopy theory of skeletal diffeological spaces. Specifically, to any smooth manifold and non-negative integer $k$, we associate a $k$-skeletal simplicial presheaf such that its $k$th cohomology with values in the circle group is isomorphic to the abelian group of Cheeger-Simons differential characters. Further, we relate these higher holonomies to the only other existing model in the literature, developed by Gajer based on the geometric loop group. The main motivation for us is to provide a model where the differential refinement is established by refining the underlying space, rather than the coefficient object. This has the advantage of possible generalizations to non-abelian differential cohomology.

==> archive.tex <==

This is the old version of the $(k-1)$-connected proof.

\begin{proposition}
    Let $(M,x_0)$ be a pointed $(k-1)$-connected smooth manifold for $k > 0$. Then there is an isomorphism of abelian groups 
    \[
    \hat{\kappa} \colon \hat{H}^{k+1}(M,\mathbb{Z}) \xrightarrow{\cong} \mathrm{Hom}_{\mathrm{PSh}(\mathbf{Cart}, \mathbf{Ab})} \left(  G^{k}(M) , U(1)   \right)
    \]
\end{proposition}
\begin{proof}
The proof of this result follows as an adaptation of the proof of Theorem \ref{Theorem: Gajer's holonomy Theorem} which is Theorem 4.2 in \cite{GajerHigher}. As shown in the general case, any differential character $\chi \in \hat{H}^k(M;\mathbb{Z})$ considered as morphism of abelian groups $\chi \colon \tilde{Z}_k(M) \rightarrow U(1)$ gives rise to a smooth morphism of abelian groups $G^{k-1}(A(M)) \rightarrow U(1)$ via precomposition with a morphism $\kappa \colon G^{k-1}(A(M)) \rightarrow \tilde{Z}_k(M)$. Notice that here $\tilde{Z}_k(M)$ denotes the abelian group obtained by a quotient of the abelian group of geometric cycles in $M$. For a detailed account on how to represent singular homology classes via geometric chains using stratifolds, see \cite{Kreck}. In particular, we can restrict this morphism further along the natural smooth map $G^{k}(M) \rightarrow G^{k-1}(A(M))$ to obtain a smooth map $G^{k}(M) \rightarrow U(1)$. By abuse of notation, we call the composition $G^{k}(M) \rightarrow G^{k-1}(A(M)) \xrightarrow{\kappa} U(1)$ also $\kappa$. This defines a morphism of abelian groups 
\[
\hat{\kappa} \colon \hat{H}^k(M,\mathbb{Z}) \rightarrow \mathrm{Hom}_{\mathbf{DiffGrp}}\left( G^{k}(M), U(1) \right). 
\]
To show that $\hat{\kappa}$ is indeed an isomorphism, we need to show that for every smooth morphism $h \colon G^{k}(M) \rightarrow U(1)$, there is a unique extension $\tilde{h} \colon \tilde{Z}_k(M) \rightarrow U(1)$ which is an element of $\hat{H}^k(M,\mathbb{Z})$. Since $M$ is $(k-1)$-connected it follows that $\kappa_* \colon \pi_0\left( G^{k}(M) \right) \xrightarrow{\cong} \tilde{H}_k(M,\mathbb{Z})$. Here the geometric homology group $\tilde{H}_k(M,\mathbb{Z}) = \tilde{Z}_k(M)/\tilde{B}_k(M)$ is naturally isomorphic to the usual singular homology of $M$. \\

It follows from this fact that for every $\xi \in \tilde{Z}_k(M)$ there is some $\gamma \in G^{k}(M)$ and $\partial \eta \in \tilde{B}_k(M)$ satisfying 
\[
\xi = \kappa(\gamma) + \partial \eta
\]
Now any extension $\tilde{h} \colon \tilde{Z}_k(M) \rightarrow U(1)$ of $h$ along $\kappa$ evaluated at $\xi$ gives 
\[
\tilde{h}(\xi) = h(\gamma) \cdot \tilde{h}(\partial \eta)
\]
An appropriate adaptation of Lemma 4.3 in \cite{GajerHigher} then shows that necessarily $\tilde{h}(\partial \eta) = \mathrm{exp} \left( 2 \pi i \int_\eta A_h \right)$ where here $A_h$ denotes the curvature form associated to the smooth map $h \colon G^{k}(M) \rightarrow U(1)$. Therefore, the equation 
\[
\tilde{h}(\xi) = h(\gamma) \cdot  \mathrm{exp} \left( 2 \pi i \int_\eta A_h \right)
\]
uniquely defines the extension $\tilde{h}$. 
\end{proof}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This is the old proof using Berwick-Evans, Boavida, Pavlov



\begin{definition}
    Let $F$ be a simplicial presheaf on $\mathbf{Mfd}$. Then define the simplicial presheaf $\mathbf{B}F$ on $\mathbf{Mfd}$ as follows: 
    \[
    \mathbf{B}F(M) := \delta \left( F( M \times \mathbb{A}^{\bullet})_{\bullet} \right) 
    \]
    where $\delta$ is the diagonal simplicial set functor 
    \[
    \delta \colon \mathbf{sSp} \rightarrow \mathbf{sSet}
    \]
    sending a bisimplicial set $K_{\bullet,\bullet}$ to its diagonal simplicial set $\delta(K)_n = K_{n,n}$.
\end{definition}
\begin{remark}
    Notice that in the case where $X$ is a diffeological space considered as a simplicial presheaf on $\mathbf{Mfd}$ that is discrete in the simplicial direction we have that 
    \[
    \mathbf{B}X(M)_n = X(M \times \mathbb{A}^n) = C^{\infty}(M \times \mathbb{A}^n,X) \cong C^{\infty}(\mathbb{A}^n, D(M,X))
    \]
    It therefore follows that 
    \[
    \mathbf{B}X(M) \cong S_e(C^{\infty}(M,X)) = \overline{X}(M)
    \]
    Since this identification is natural in $M$ the simplicial presheaf $\mathbf{B}X$ is isomorphic to the enriched presheaf $\overline{X}$. 
\end{remark}





\begin{theorem}[Theorem 1.1 \cite{BBP}] \label{Theorem: Classifying space for infinity sheaf}
    Let $F$ be an $\infty$-sheaf on $\mathbf{Mfd}$. Then there is an evaluation map 
    \[
    \mathbf{B}F(M) \rightarrow \mathrm{Map}(S_e(M),BF)
    \]
    which is a natural weak equivalence of spaces for every manifold $M$. Here the classifying space $BF$ is given by a fibrant replacement of the simplicial set $\mathbf{B}F(*)$. 
\end{theorem}



Let us for a moment have a look at the site of manifolds $\mathbf{Mfd}$ where the covering families are given by open coverings. 

\begin{definition}
    Let $\mathbf{Mfd}$ denote the category of finite-dimensional smooth manifolds without boundary and smooth maps. The \textbf{coverage of open covers} on the category $\mathbf{Mfd}$ is the function assigning to every object $M \in \mathbf{Mfd}$ the collection of covering families given by open coverings of $M$. That is for every $M$ let $\cat{I}(M)$ denote the collection of open covers of $M$. The category $\mathbf{Mfd}$ together with this coverage defines the site $(\mathbf{Mfd}, \tau_{\mathrm{open}})$.   
\end{definition}

Recall that the standard coverage on the category $\mathbf{Cart}$ is set to be the one given by goop open coverings and the site is denoted by $(\mathbf{Cart}, \tau_{\mathrm{gd}})$. The \textit{comparison lemma} allows us to identify sheaves on the site  $(\mathbf{Mfd}, \tau_{\mathrm{open}})$ with sheaves on the site $(\mathbf{Cart}, \tau_{\mathrm{gd}})$ along the subcategory inclusion $\mathbf{Cart} \hookrightarrow \mathbf{Mfd}$. 

\begin{proposition}[Theorem 2.2.3 \cite{Johnstone}] \label{Proposition: Comparison Lemma}
    Let $(\cat{C},\tau)$ be a site with a Grothendieck coverage and $\cat{C}' \hookrightarrow \cat{C}$ a $\tau$-dense full subcategory. Then the restriction functor $\mathrm{res} \colon \mathrm{PSh}(\cat{C}) \rightarrow \mathrm{PSh}(\cat{C}')$ restricts to an equivalence of categories
    \[
    \mathrm{res} \colon \mathrm{Sh}(\cat{C},\tau) \rightarrow \mathrm{Sh}(\cat{C}',\tau|_{\cat{C}'})
    \]
\end{proposition}

\begin{corollary} \label{Corollary: Comparison Lemma applied}
   The restriction functor from Proposition \ref{Proposition: Comparison Lemma} induces an equivalence of categories 
   \[
   \mathrm{res} \colon \mathrm{Sh}(\mathbf{Mfd},\tau_{\mathrm{open}}) \xrightarrow{\simeq} \mathrm{Sh}(\mathbf{Cart},\tau_{\mathrm{gd}})
   \]
   which further restricts to an equivalence between the corresponding subcategories of concrete sheaves
   \[
   \mathrm{CSh}(\mathbf{Mfd},\tau_{\mathrm{open}}) \simeq \mathrm{CSh}(\mathbf{Cart},\tau_{\mathrm{gd}})
   \]
\end{corollary}

\begin{remark} \label{Remark: Diffeological Space is Infinity Sheaf}
    The notion of an $\infty$-sheaf appearing in Theorem \ref{Theorem: Classifying space for infinity sheaf} is defined to be a simplicial presheaf $F \in \mathrm{sPSh}(\mathbf{Mfd})$ satisfying \v{C}ech descent with respect to the coverage given by open coverings $\tau_{\mathrm{open}}$. In particular fibrant objects in the \v{C}ech-local model structures provide examples of such $\infty$-sheaves. As such, notice that by Corollary \ref{Corollary: Comparison Lemma applied} any diffeological space $X$ considered as a concrete sheaf on the site $(\mathbf{Mfd},\tau_{\mathrm{open}})$ defines an $\infty$-sheaf via the standard fully faithful inclusion into simplicial presheaves on $\mathbf{Mfd}$.  
\end{remark}


\begin{corollary}
    Let $X$ be a fibrant diffeological space. Then the evaluation map of Theorem \ref{Theorem: Classifying space for infinity sheaf} induces a morphism of simplicial presheaves on $\mathbf{Cart}$
    \[
    \overline{X}(-) \rightarrow \mathrm{Map}(S_e(-),S_e(X))
    \]
    between the enriched simplicial presheaf $\overline{X}$ associated with $X$ and the simplicial presheaf given by 
    \[
    U \mapsto \mathrm{Map}(S_e(U),S_e(X)) 
    \]
    In particular, this is an objectwise weak equivalence of simplicial presheaves on $\mathbf{Cart}$. 
\end{corollary}
\begin{proof}
    Since $X$ is a diffeological space, it defines a simplicial presheaf on $\mathbf{Mfd}$ that is discrete in the simplicial direction. By Remark \ref{Remark: Diffeological Space is Infinity Sheaf} it follows that this simplicial presheaf is infact an $\infty$-sheaf after \cite{BBP}.  As we have seen earlier there is an isomorphism of simplicial presheaves 
    \[
    \mathbf{B}X \cong \overline{X}
    \]
    which in particular shows that by evaluating on the point we get that the smooth singular complex is a model for the classifying space of $X$, since we assumed $X$ to be fibrant.  
    \[
    BX = S_e(X)  \cong  \mathbf{B}X(*) 
    \]
    The natural weak equivalence from Theorem \ref{Theorem: Classifying space for infinity sheaf} now induces the desired objectwise weak equivalence of simplicial presheaves.  
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

This is the old change of orientation operator

To prove this Proposition we recall the construction of the \textit{prism operator} for singular chains. The idea behind this operator is to subdivide the product $|\Delta^{k}| \times |\Delta^1|$ into $(k+1)$-simplices. In order to define the prism operator denote $|\Delta^{k}| \times \{0\} = [v_0, ..., v_{k}]$ and $|\Delta^k| \times \{1\} = [w_0, ..., w_{k}]$ such that $w_i$ and $v_i$ have the same image under the smooth projection map $\pi \colon |\Delta^{k}| \times |\Delta^1| \rightarrow |\Delta^{k}|$. Define now the operator $P \colon C_{k}(X) \rightarrow C_{k+1}(X)$ by 
\[
P(\eta) := \sum_{i = 0}^{k} (-1)^i (\eta \circ \pi)|_{[v_0, ..., v_i, w_i, ..., w_{k}]}
\]
for $\eta \colon |\Delta^{k}| \rightarrow X$ some smooth simplex in $X$. \\




For a finite set $X$ denote by $S_X$ the symmetric group on $X$. Since we are primarily interested in permutations of vertices of simplicies we write $S_{k+1}:= S_{\{0,...,k\}}$ for all $k \geq 0$ so that a permutation $\sigma \in S_{k+1}$ always acts on the set $[k] = \{0,...,k\}$. Given a permutation $\sigma \in S_{k+1}$ and $S \subset \{0,..,k\}$ a non-empty subset, the restriction $\sigma|_{S} \colon S \rightarrow \sigma(S)$ gives an isomorphism of sets. The total order of $\mathbb{N}$ uniquely determines isomorphisms $\varphi_S \colon \{ 1, ..., |S|\} \xrightarrow{\cong} S$ and $\psi_S \colon \{1,...,|S|\} \xrightarrow{\cong} \sigma(S)$ which are order preserving. Then, the \textit{induced permutation on} $S$, denoted $\tilde{\sigma}_S$ is then given by: 
\begin{center}
    \begin{tikzcd}
S \arrow[r, "\sigma|_S"]                                   & \sigma(S) \arrow[d, "\psi"] \\
{\{ 0,...,|S|-1\}} \arrow[u, "\varphi"] \arrow[r, "\tilde{\sigma}_S"'] & {\{ 0,...,|S|-1\}}            
\end{tikzcd}
\end{center}
In particular one has $\sigma_S \in S_{|S|}$. Sometimes, however, we wish to regard $\tilde{\sigma}_S$ as a permutation of $S$ itself and we set $\sigma_S = \varphi_S \circ \tilde{\sigma}_S \circ \varphi_S^{-1}$. This also allows to define the signauture of $\sigma_S$ via $\mathrm{sgn}(\sigma_S):= \mathrm{sgn}(\tilde{\sigma}_S)$. 
\begin{example}
    Let $\sigma \in S_4$ be the permutation given by $\sigma = (0132)$ and $S \subset \{0,1,2,3\}$ be the subset $S = \{0,1,3\}$. Then the permutation $\sigma_S \in S_3$ is given by $\sigma_S = (12)$. Indeed, $\sigma(S) = \{ 1,2,3 \}$ such that then we have that 
    \begin{align*}
    \sigma_S(0) =  \psi(\sigma( \varphi(0))) = \psi( \sigma(0) ) = \psi(1) = 0 \\
    \sigma_S(1) =  \psi(\sigma( \varphi(1))) = \psi( \sigma(1) ) = \psi(3) = 2 \\
    \sigma_S(2) =  \psi \sigma( \varphi(2))) = \psi( \sigma(3) ) = \psi(2) = 1
    \end{align*}
\end{example}

For every $\sigma \in S_{k+1}$ we now define the \textit{adjusted prism operator} $P_{\sigma} \colon C_{k}(X) \rightarrow C_{k+1}(X)$ by 
\[
P_{\sigma}(\eta) := \sum_{j = 0}^{k} (-1)^j \mathrm{sgn}(\sigma_j) (\eta \circ \pi)|_{[v_0, ..., v_j, w_{\sigma_{j}(j)}, ..., w_{\sigma_j(k)}]}
\]
for $\eta \colon |\Delta^{k}| \rightarrow X$ some smooth simplex in $X$. Notice that here $\sigma_j:= \sigma_{\{j,...,k\}}$ considered as a permutation of $\{j,...,k\}$. Notice that in the case $j = 0$ of course it follows $\sigma_0 = \sigma$ and $\sigma_k = \mathrm{id}_{\{k\}}$. 


\begin{definition}
    Given $\sigma \in S_{k+1}$ a permutation with $\sigma(0) = 0$, define the \textbf{change of orientation operator} $D_{\sigma} \colon C^{\Delta}_{k}(M) \rightarrow C^{\Delta}_{k}(M)$ by 
    \[
    D_{\sigma}(\eta) := \sum_{i = 0}^{k} (-1)^i P_{\tilde{\sigma}^i} \left( \eta|_{[v_0, ..., \hat{v_i}, ..., v_k]} \right) 
    \]
    where we denote by $\tilde{\sigma}^i$ the induced permutation $\tilde{\sigma}_{\{0,...,\hat{i},...,k\}} \in S_{k}$ omitting the $i$-th vertex. 
\end{definition}

\begin{remark}
Omitting the terms $(\eta \circ \pi)$ for better readability the change of orientation operator is given by:
    \begin{align*} \label{Equation: Permutation Formula}
    D_{\sigma}(\eta) &= \sum_{0 \leq i < j \leq k}  (-1)^{i+j-1} \mathrm{sgn}(\sigma_j) [v_0, ..., \widehat{v_i}, ..., v_j, w_{\sigma_j(j)}, ..., w_{\sigma_j(k)}] \\
    &+ \sum_{0 \leq j < i \leq k}  (-1)^{i+j} \mathrm{sgn}\left( \sigma_{\{j, ..., \hat{i}, ...,k\}} \right) [v_0, ..., v_j, w_{\sigma_j(j)}, ..., \widehat{w_{\sigma_j(i)}}, ..., w_{\sigma_j(k)}]
    \end{align*}

\end{remark}




The change of orientation operator is such that for any $\eta \in C^{\Delta}_{k+1}(M)$ and $\sigma \in S_{k+2}$ with $\sigma(0) =0$ on has that 
\[
\partial D_{\sigma}(\eta) = \mathrm{sgn}(\sigma) \partial(\eta \circ \sigma) - \partial(\eta) 
\]
By construction of $D_{\sigma}$ if follows that for $\eta \in C^{\Delta}_{k+1}(M)$ the image $D_{\sigma}(\eta) \in C^{\Delta}_{k+1}(M_k)$, which then in particular implies that 
\[
\mathrm{sgn}(\sigma) \cdot \left[ \partial(\eta \circ \sigma) \right]_k = \left[ \partial(\eta)   \right]_k
\]



\begin{example}
The geometric meaning behind the change of orientation operator is observed best by looking at an example. Let therefore $\eta \colon |\Delta^2| \rightarrow M$ be a smooth simplex and consider the permutation $\sigma = (12) \in S_3$. We now want to compute $D_{\sigma}(\eta) \in C^{\Delta}_{2}(M)$. For notational reasons denote $[v_0,v_1,v_2] = |\Delta^2|$ and we omit $\eta$ and $\pi$ in the formulas. Now by definition one has 
\[
D_{\sigma}([v_0,v_1,v_2]) = P_{\tilde{\sigma}^0}([v_1,v_2]) - P_{\tilde{\sigma}^1}([v_0,v_2]) + P_{\tilde{\sigma}^2}([v_0,v_1])
\]
Let us have a look at the induced permutations $\tilde{\sigma}^i \in S_2$ for $0 \leq i \leq 2$ first. One computes that $\tilde{\sigma}^0 = (01)$, $\tilde{\sigma}^1 = \mathrm{id}$ and $\tilde{\sigma}^2 = \mathrm{id}$. Before we continue with the computation, notice that for each $i$ the adjusted Prism operator $P_{\tilde{\sigma}^i}([v_0, ..., \hat{v_i}, .., v_2])$ corresponds to the prism operator of the $i$-th square in the diagram 
\begin{center}
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,414); %set diagram left start at 0, and has height of 414

%Straight Lines [id:da4128468269902479] 
\draw    (96,208) -- (244,208) ;
\draw [shift={(244,208)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.01, y radius= 2.01]   ;
\draw [shift={(173.6,208)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-2.94) .. controls (4.17,-1.38) and (1.99,-0.4) .. (0,0) .. controls (1.99,0.4) and (4.17,1.38) .. (6.56,2.94)   ;
\draw [shift={(96,208)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.01, y radius= 2.01]   ;
%Straight Lines [id:da38501338744580504] 
\draw    (96,208) -- (196,144) ;
\draw [shift={(196,144)}, rotate = 327.38] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.01, y radius= 2.01]   ;
\draw [shift={(149.03,174.06)}, rotate = 147.38] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-2.94) .. controls (4.17,-1.38) and (1.99,-0.4) .. (0,0) .. controls (1.99,0.4) and (4.17,1.38) .. (6.56,2.94)   ;
\draw [shift={(96,208)}, rotate = 327.38] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.01, y radius= 2.01]   ;
%Straight Lines [id:da3196725764248247] 
\draw    (244,208) -- (196,144) ;
\draw [shift={(196,144)}, rotate = 233.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.01, y radius= 2.01]   ;
\draw [shift={(217.84,173.12)}, rotate = 53.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-2.94) .. controls (4.17,-1.38) and (1.99,-0.4) .. (0,0) .. controls (1.99,0.4) and (4.17,1.38) .. (6.56,2.94)   ;
\draw [shift={(244,208)}, rotate = 233.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.01, y radius= 2.01]   ;
%Straight Lines [id:da4145836829538896] 
\draw    (96,116) -- (244,116) ;
\draw [shift={(244,116)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.01, y radius= 2.01]   ;
\draw [shift={(173.6,116)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-2.94) .. controls (4.17,-1.38) and (1.99,-0.4) .. (0,0) .. controls (1.99,0.4) and (4.17,1.38) .. (6.56,2.94)   ;
\draw [shift={(96,116)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.01, y radius= 2.01]   ;
%Straight Lines [id:da3839969507945242] 
\draw    (96,116) -- (196,52) ;
\draw [shift={(196,52)}, rotate = 327.38] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.01, y radius= 2.01]   ;
\draw [shift={(149.03,82.06)}, rotate = 147.38] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-2.94) .. controls (4.17,-1.38) and (1.99,-0.4) .. (0,0) .. controls (1.99,0.4) and (4.17,1.38) .. (6.56,2.94)   ;
\draw [shift={(96,116)}, rotate = 327.38] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.01, y radius= 2.01]   ;
%Straight Lines [id:da15067317289725857] 
\draw    (196,52) -- (244,116) ;
\draw [shift={(244,116)}, rotate = 53.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.01, y radius= 2.01]   ;
\draw [shift={(222.16,86.88)}, rotate = 233.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-2.94) .. controls (4.17,-1.38) and (1.99,-0.4) .. (0,0) .. controls (1.99,0.4) and (4.17,1.38) .. (6.56,2.94)   ;
\draw [shift={(196,52)}, rotate = 53.13] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.01, y radius= 2.01]   ;
%Straight Lines [id:da25922965606113646] 
\draw    (96,116) -- (96,208) ;
\draw [shift={(96,157.4)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-2.94) .. controls (4.17,-1.38) and (1.99,-0.4) .. (0,0) .. controls (1.99,0.4) and (4.17,1.38) .. (6.56,2.94)   ;
%Straight Lines [id:da6284085148759058] 
\draw    (196,52) -- (196,144) ;
\draw [shift={(196,93.4)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-2.94) .. controls (4.17,-1.38) and (1.99,-0.4) .. (0,0) .. controls (1.99,0.4) and (4.17,1.38) .. (6.56,2.94)   ;
%Straight Lines [id:da8190577940403758] 
\draw    (244,116) -- (244,208) ;
\draw [shift={(244,157.4)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (6.56,-2.94) .. controls (4.17,-1.38) and (1.99,-0.4) .. (0,0) .. controls (1.99,0.4) and (4.17,1.38) .. (6.56,2.94)   ;

% Text Node
\draw (85,212.4) node [anchor=north west][inner sep=0.75pt]    {$v_{0}$};
% Text Node
\draw (233,210.4) node [anchor=north west][inner sep=0.75pt]    {$v_{1}$};
% Text Node
\draw (185,154.4) node [anchor=north west][inner sep=0.75pt]    {$v_{2}$};
% Text Node
\draw (69,106.4) node [anchor=north west][inner sep=0.75pt]    {$w_{0}$};
% Text Node
\draw (253,108.4) node [anchor=north west][inner sep=0.75pt]    {$w_{1}$};
% Text Node
\draw (189,26.4) node [anchor=north west][inner sep=0.75pt]    {$w_{2}$};


\end{tikzpicture}
\end{center}
where the $i$-th square denotes the square opposite the edge $[v_i,w_i]$. The permutation $\sigma$ induces an ordering of the upper vertices $\{w_0,w_1,w_2\}$, and in each square the ordering of the upper vertices corresponds to $\tilde{\sigma}^i$. Indeed, in the $0$-th square the order is changed which corresponds to $\tilde{\sigma}^0 = (01)$ whereas in the remaining squares, the order stays unchanged. \\

By definition of the adjusted prism operator, it follows
\[
P_{\tilde{\sigma}^0}([v_1,v_2]) =  \mathrm{sgn}(\sigma^0_0)[v_1,w_{2},w_{1}] - \mathrm{sgn}(\sigma^0_1)[v_1,v_2,w_{2}] =          -[v_1,w_2,w_1] - [v_1,v_2,w_2]
\]
using that $\sigma^0_0 = \sigma^0 = (12)$ and $\sigma^0_1 \in S_1$ hence is the identity. Likewise one computes 

\[
P_{\tilde{\sigma}^2}([v_0,v_1]) = [v_0,w_{0},w_{1}] - [v_0,v_1,w_{1}]
\]
and
\[
P_{\tilde{\sigma}^1}([v_0,v_2]) = [v_0,w_{0},w_{2}] - [v_0,v_2,w_{2}]. 
\]
This then gives 

\[
D_{\sigma}([v_0,v_1,v_2]) = -[v_1,w_2,w_1] - [v_1,v_2,w_2] - [v_0,w_{0},w_{2}] + [v_0,v_2,w_{2}] + [v_0,w_{0},w_{1}] - [v_0,v_1,w_{1}]
\]
and a simple computation leads to
\[
\partial(D_{\sigma}([v_0,v_1,v_0])) = \mathrm{sgn}(\sigma)\partial[w_{\sigma(0)},w_{\sigma(1)},w_{\sigma(2)}] - \partial[v_0,v_1,v_2]  = -\partial[w_0,w_2,w_1] - \partial[v_0,v_1,v_2].
\]
\end{example}




\begin{proof}[Proof of Proposition \ref{Proposition: Change of Orientation}]
    Let $M$ be a smooth manifold and $\eta \colon |\Delta^{k+1}| \rightarrow M$ a smooth $(k+1)$-simplex in $M$ and $\sigma \in S_{k+2}$ a permutation such that $\sigma(0) = 0$. The idea is to use the change of orientation operator $D_{\sigma} \colon C_{k+1}^{\Delta}(M) \rightarrow C_{k+1}^{\Delta}(M)$. More preciesly, we claim that 
    \[
    \partial D_{\sigma}(\eta) =  \mathrm{sgn}(\sigma) \partial(\eta \circ \sigma) - \partial(\eta) 
    \]
    Also, notice that by construction $D_{\sigma}(\eta) \in C_{k+1}^{\Delta}(M_k)$ since we are taking the sum over the adjusted prism operators of the boundary components. Since each adjusted prism operator itself is given by a sum of simplices involving the projection $\pi$ it follows that each smooth simplex in the chain $D_{\sigma}(\eta)$ factors trough $\eta|_{[v_0, ..., \hat{v_i}, ..., v_{k+1}]}$, i.e. a $|\Delta^{k}|$-simplex and therefore $D_{\sigma}(\eta) \in C_{k+1}^{\Delta}(M_k)$. It then follows from the earlier claim that
    \[
    \left[  \mathrm{sgn}(\sigma) \partial(\eta \circ \sigma) - \partial(\eta) \right]_k = 0 \in H^{\Delta}_k(M_k)
    \]
    and therefore
    \[
     \mathrm{sgn}(\sigma) \left[ \partial(\eta \circ \sigma)\right]_k = \left[\partial(\eta) \right]_k
    \]
    We are therefore left to show that
    \[
    \partial D_{\sigma}(\eta) =  \mathrm{sgn}(\sigma) \partial(\eta \circ \sigma) - \partial(\eta) 
    \]
\end{proof}

Reduce the proof to adjacent transpositions of the form $\sigma = (a a+1)$ for $a \in \{0,...,k-1\}$. Then by definition, the permutation operator is given by 
\begin{align*}
D_{\sigma}(\eta) :=& \sum_{i = 0}^{k} (-1)^i P_{\tilde{\sigma}^i} \left( \eta|_{[v_0, ..., \hat{v_i}, ..., v_k]} \right) \\
=&   \sum_{i < a} (-1)^i P_{\tilde{\sigma}^i} \left( \eta|_{[v_0, ..., \hat{v_i}, ..., v_k]} \right) +  \sum_{a \leq i \leq a+1} (-1)^i P_{\tilde{\sigma}^i} \left( \eta|_{[v_0, ..., \hat{v_i}, ..., v_k]} \right) \\
&+  \sum_{i > a +1} (-1)^i P_{\tilde{\sigma}^i} \left( \eta|_{[v_0, ..., \hat{v_i}, ..., v_k]} \right)
\end{align*}
Let us compute the induced permutations in the cases $i< a$, $a \leq i \leq a+1$ and $i > a+1$. That is, for $j \in \{0,...,\hat{i},...,k\}$ it follows
\[
\sigma^i(j) = 
\begin{cases}
\sigma(j) \text{ for } i < a \\
j  \text{ for } a \leq i \leq a + 1 \\
\sigma(j) \text{ for } i > a + 1
\end{cases}
\]



\begin{center}
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,414); %set diagram left start at 0, and has height of 414

%Straight Lines [id:da6221790420077797] 
\draw    (320,0) -- (320,368) ;
%Straight Lines [id:da23017138848191498] 
\draw    (0,48) -- (656,48) ;
%Straight Lines [id:da9649995544542156] 
\draw    (57.07,101.5) -- (119.93,101.5) ;
\draw [shift={(119.93,101.5)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
\draw [shift={(92.7,101.5)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (7.65,-3.43) .. controls (4.86,-1.61) and (2.31,-0.47) .. (0,0) .. controls (2.31,0.47) and (4.86,1.61) .. (7.65,3.43)   ;
\draw [shift={(57.07,101.5)}, rotate = 0] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
%Shape: Arc [id:dp5858345598767647] 
\draw  [draw opacity=0] (368,120) .. controls (368,89.07) and (393.07,64) .. (424,64) .. controls (454.93,64) and (480,89.07) .. (480,120) -- (424,120) -- cycle ; \draw   (368,120) .. controls (368,89.07) and (393.07,64) .. (424,64) .. controls (454.93,64) and (480,89.07) .. (480,120) ;  
%Shape: Arc [id:dp5348101090300905] 
\draw  [draw opacity=0] (480,120) .. controls (480,150.93) and (454.93,176) .. (424,176) .. controls (393.07,176) and (368,150.93) .. (368,120) -- (424,120) -- cycle ; \draw   (480,120) .. controls (480,150.93) and (454.93,176) .. (424,176) .. controls (393.07,176) and (368,150.93) .. (368,120) ;  
%Shape: Arc [id:dp8412984359589151] 
\draw  [draw opacity=0][dash pattern={on 0.84pt off 2.51pt}] (368,120) .. controls (368,120) and (368,120) .. (368,120) .. controls (368,127.73) and (393.07,134) .. (424,134) .. controls (454.93,134) and (480,127.73) .. (480,120) -- (424,120) -- cycle ; \draw  [dash pattern={on 0.84pt off 2.51pt}] (368,120) .. controls (368,120) and (368,120) .. (368,120) .. controls (368,127.73) and (393.07,134) .. (424,134) .. controls (454.93,134) and (480,127.73) .. (480,120) ;  
%Shape: Arc [id:dp3980850253115926] 
\draw  [draw opacity=0][dash pattern={on 0.84pt off 2.51pt}] (480,120) .. controls (480,120) and (480,120) .. (480,120) .. controls (480,112.27) and (454.93,106) .. (424,106) .. controls (393.07,106) and (368,112.27) .. (368,120) -- (424,120) -- cycle ; \draw  [dash pattern={on 0.84pt off 2.51pt}] (480,120) .. controls (480,120) and (480,120) .. (480,120) .. controls (480,112.27) and (454.93,106) .. (424,106) .. controls (393.07,106) and (368,112.27) .. (368,120) ;  
%Curve Lines [id:da19053799027633733] 
\draw    (412,160) .. controls (475.75,141) and (402.25,130.5) .. (432,80) ;
\draw [shift={(432,80)}, rotate = 300.5] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
\draw [shift={(412,160)}, rotate = 343.4] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
%Shape: Arc [id:dp29187412962543813] 
\draw  [draw opacity=0] (368,280) .. controls (368,249.07) and (393.07,224) .. (424,224) .. controls (454.93,224) and (480,249.07) .. (480,280) -- (424,280) -- cycle ; \draw   (368,280) .. controls (368,249.07) and (393.07,224) .. (424,224) .. controls (454.93,224) and (480,249.07) .. (480,280) ;  
%Shape: Arc [id:dp9508033241509037] 
\draw  [draw opacity=0] (480,280) .. controls (480,310.93) and (454.93,336) .. (424,336) .. controls (393.07,336) and (368,310.93) .. (368,280) -- (424,280) -- cycle ; \draw   (480,280) .. controls (480,310.93) and (454.93,336) .. (424,336) .. controls (393.07,336) and (368,310.93) .. (368,280) ;  
%Shape: Arc [id:dp584912797616421] 
\draw  [draw opacity=0][dash pattern={on 0.84pt off 2.51pt}] (368,280) .. controls (368,280) and (368,280) .. (368,280) .. controls (368,287.73) and (393.07,294) .. (424,294) .. controls (454.93,294) and (480,287.73) .. (480,280) -- (424,280) -- cycle ; \draw  [dash pattern={on 0.84pt off 2.51pt}] (368,280) .. controls (368,280) and (368,280) .. (368,280) .. controls (368,287.73) and (393.07,294) .. (424,294) .. controls (454.93,294) and (480,287.73) .. (480,280) ;  
%Shape: Arc [id:dp23222558091232104] 
\draw  [draw opacity=0][dash pattern={on 0.84pt off 2.51pt}] (480,280) .. controls (480,280) and (480,280) .. (480,280) .. controls (480,272.27) and (454.93,266) .. (424,266) .. controls (393.07,266) and (368,272.27) .. (368,280) -- (424,280) -- cycle ; \draw  [dash pattern={on 0.84pt off 2.51pt}] (480,280) .. controls (480,280) and (480,280) .. (480,280) .. controls (480,272.27) and (454.93,266) .. (424,266) .. controls (393.07,266) and (368,272.27) .. (368,280) ;  
%Curve Lines [id:da1694014694408601] 
\draw    (412,320) .. controls (475.75,301) and (402.25,290.5) .. (432,240) ;
\draw [shift={(432,240)}, rotate = 300.5] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
\draw [shift={(412,320)}, rotate = 343.4] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
%Curve Lines [id:da17653361265516665] 
\draw    (45.31,284) .. controls (71.02,238) and (120.18,247) .. (136.33,284) ;
\draw [shift={(136.33,284)}, rotate = 66.41] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
\draw [shift={(95.45,252.95)}, rotate = 181.27] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (7.65,-3.43) .. controls (4.86,-1.61) and (2.31,-0.47) .. (0,0) .. controls (2.31,0.47) and (4.86,1.61) .. (7.65,3.43)   ;
\draw [shift={(45.31,284)}, rotate = 299.21] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
%Curve Lines [id:da5440538591903701] 
\draw    (45.31,284) .. controls (68.75,323.5) and (109.71,330.5) .. (136.33,284) ;
\draw [shift={(136.33,284)}, rotate = 299.79] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
\draw [shift={(95.58,316.1)}, rotate = 178.52] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (7.65,-3.43) .. controls (4.86,-1.61) and (2.31,-0.47) .. (0,0) .. controls (2.31,0.47) and (4.86,1.61) .. (7.65,3.43)   ;
\draw [shift={(45.31,284)}, rotate = 59.32] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
%Curve Lines [id:da6478295329295751] 
\draw    (412,320) .. controls (419.25,280.5) and (362.75,254) .. (432,240) ;
\draw [shift={(432,240)}, rotate = 348.57] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
\draw [shift={(412,320)}, rotate = 280.4] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 2.34, y radius= 2.34]   ;
%Curve Lines [id:da8099429220059855] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (156.25,155) .. controls (196.23,186.69) and (172.03,210.29) .. (155.04,224.89) ;
\draw [shift={(153.75,226)}, rotate = 319.54] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Curve Lines [id:da3944220339701201] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (504.25,155) .. controls (544.23,186.69) and (520.03,210.29) .. (503.04,224.89) ;
\draw [shift={(501.75,226)}, rotate = 319.54] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (128,18) node [anchor=north west][inner sep=0.75pt]   [align=left] {Structure};
% Text Node
\draw (381,17) node [anchor=north west][inner sep=0.75pt]   [align=left] {Physical/Geometric Interpretation};
% Text Node
\draw (39,91.9) node [anchor=north west][inner sep=0.75pt]    {$x$};
% Text Node
\draw (129,91.9) node [anchor=north west][inner sep=0.75pt]    {$y$};
% Text Node
\draw (80.71,109.4) node [anchor=north west][inner sep=0.75pt]    {$\gamma $};
% Text Node
\draw (529,105.4) node [anchor=north west][inner sep=0.75pt]    {$ \begin{array}{l}
\mathrm{Points:} \ x,y\\
\mathrm{Paths:} \ \gamma 
\end{array}$};
% Text Node
\draw (513,258.4) node [anchor=north west][inner sep=0.75pt]    {$ \begin{array}{l}
\mathrm{Points:} \ x,y\\
\mathrm{Paths:} \ \gamma ,\gamma '\\
\mathrm{Surfaces:} \ \Sigma 
\end{array}$};
% Text Node
\draw (84,273.4) node [anchor=north west][inner sep=0.75pt]  [font=\large]  {$\Downarrow $};
% Text Node
\draw (24.37,276.4) node [anchor=north west][inner sep=0.75pt]    {$x$};
% Text Node
\draw (145.63,274.9) node [anchor=north west][inner sep=0.75pt]    {$y$};
% Text Node
\draw (87.56,231.9) node [anchor=north west][inner sep=0.75pt]    {$\gamma $};
% Text Node
\draw (84.02,325.4) node [anchor=north west][inner sep=0.75pt]    {$\gamma '$};
% Text Node
\draw (177,256) node [anchor=north west][inner sep=0.75pt]   [align=left] {objects: $\displaystyle x,y$\\1-morphisms: $\displaystyle \gamma ,\gamma '$\\2-morphisms: $\displaystyle \Sigma $$ $};
% Text Node
\draw (177,82) node [anchor=north west][inner sep=0.75pt]   [align=left] {objects: $\displaystyle x,y$\\morphisms: $\displaystyle \gamma $};
% Text Node
\draw (465,334.4) node [anchor=north west][inner sep=0.75pt]    {$M$};
% Text Node
\draw (465,174.4) node [anchor=north west][inner sep=0.75pt]    {$M$};
% Text Node
\draw (394,147.9) node [anchor=north west][inner sep=0.75pt]    {$x$};
% Text Node
\draw (413,72.4) node [anchor=north west][inner sep=0.75pt]    {$y$};
% Text Node
\draw (436,112.9) node [anchor=north west][inner sep=0.75pt]    {$\gamma $};
% Text Node
\draw (393.5,310.9) node [anchor=north west][inner sep=0.75pt]    {$x$};
% Text Node
\draw (437.5,232.4) node [anchor=north west][inner sep=0.75pt]    {$y$};
% Text Node
\draw (386.5,271.4) node [anchor=north west][inner sep=0.75pt]    {$\gamma $};
% Text Node
\draw (441,272.4) node [anchor=north west][inner sep=0.75pt]    {$\gamma '$};
% Text Node
\draw (409,270.9) node [anchor=north west][inner sep=0.75pt]    {$\Sigma $};
% Text Node
\draw (68.5,274.4) node [anchor=north west][inner sep=0.75pt]    {$\Sigma $};
% Text Node
\draw (187.5,179) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textcolor[rgb]{0.82,0.01,0.11}{categorification}};
% Text Node
\draw (535.5,179) node [anchor=north west][inner sep=0.75pt]   [align=left] {\textcolor[rgb]{0.82,0.01,0.11}{categorification}};

\end{tikzpicture}
\end{center}
This categorification procedure goes on, which gives rise to higher path groupoids, higher bundles with connection, etc. Say something about why it makes sense to model quantum particles and their time evolution by paths and integrals over such paths. This relies on Feynman's path integral approach \cite{Baez-Huerta}.   
